Wasserstein-Splitting Gaussian Process Regression for Heterogeneous Online Bayesian Inference

Gaussian processes (GPs) are a well-known nonparametric Bayesian inference technique, but they suffer from scalability problems for large sample sizes, and their performance can degrade for non-stationary or spatially heterogeneous data. In this work, we seek to overcome these issues through (i) employing variational free energy approximations of GPs operating in tandem with online expectation propagation steps; and (ii) introducing a local splitting step which instantiates a new GP whenever the posterior distribution changes significantly as quantified by the Wasserstein metric over posterior distributions. Over time, then, this yields an ensemble of sparse GPs which may be updated incrementally, and adapts to locality, heterogeneity, and non-stationarity in training data.

==> Introduction.tex <==
%!TEX root = root.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Introduction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
In a wide variety of robotics applications, Gaussian process regression has been used to estimate a scalar function of interest $f:\calX\rightarrow\bbR$, with applications ranging from mapping geo-physical quantities like terrain elevation \cite{vasudevan2009gaussian} or temperature \cite{krause2008near}, to learning complex nonlinear phenomenon such as the inverse mapping of sensor outputs to joint inputs for the control of a robotic arm \cite{nguyen2009model}. In the simplest  setting, the spatial field $f$ is stationary, meaning that it can be best described using a single set of hyperparameters throughout the entire domain. In more complex settings, the spatial field need not be stationary. For example, when one region of the domain is characterized by a high level of measurement noise and another region by low noise. Intuitively, this can be addressed using a collection of Gaussian process models. Previous approaches that employ a collection of models instantiate a new model based on distance to other existing models, even if the hyperparameters of the new model are the same as an existing model. In this paper we propose a new approach to performing inference with a collection of models, where a new model is instantiated on the basis of how similar its posterior distribution is to that of an existing model.

In local Gaussian process regression (LGPR), proposed by Nguyen et al. \cite{nguyen2009model}, inference is performed using a set of Gaussian process models, where each model is associated with a particular region of the domain. New training data is assigned to a particular model based on a similarity measure. Under the assumption that inputs close in proximity are likely to have similar function values, the notion of similarity is made precise in terms of the covariance kernel used for regression. For example, when a squared-exponential kernel is used for regression then the new point is added to the model that has the largest similarity measure, with the measure of the $j^{th}$ model given by
\begin{align} \label{eq: weights}
 w_j(\bx_{new}) &\triangleq \sigma_f^2 \exp\left\{-\frac{1}{2}(\bx_{new}-\bc_j)^{\tpose}\Lambda^{-1}(\bx_{new}-\bc_j)\right\},
 \end{align}
 where $\bc_j$ is the geometric center of inputs belonging to the $j^{th}$ model, i.e. $\bc_j \triangleq \frac{1}{M_j}\sum^{M_j}_{i=1}\bx_i$. In \cite{nguyen2009model}, the hyperparameters $\theta = \{\sigma_f,\Lambda\}$ of the covariance kernel, and hence the similarity measure \eqref{eq: weights}, are fixed \textit{a priori} by optimizing the log likelihood over a subset of available training data, which is ideally characteristic of the entire domain. If no models are sufficiently close such that largest weight is less than a user-defined threshold $w_{gen}$, then the new data point is used to instantiate a new model. If a model contains the maximum number of allowable data points, LGPR requires that a new data point only be added to the local model provided the data point is sufficiently informative in terms of entropy or mutual information, which can be computed in closed form (see Krause et al. \cite{krause2008near}). The new point then replaces an old one, chosen at random, in the set.
 
 The prediction at a location of interest $\bx_s\in \calX$ is the normalized weighted average
 of the predictions of each local model, with the weights given by \eqref{eq: weights}. Nguyen et al.  \cite{nguyen2009model} report experimental results where the weighted average is taken over all models $GP_j$ that are activated, i.e. $w_j(\bx_s)>w_{gen}$. Alternatively, the weighted average can be taken over the $\hat{J} \ll J$ closest models. Nguyen et al. \cite{nguyen2009model} assert that, in practice, using the 2 or 3 models closest to the query point $\bx_s$ suffices. 
 
 In various practical applications there is no \textit{a priori} access to a dataset, characteristic of the entire domain, to learn the hyperparameters of the similarity measure and covariance kernel. Instead methods, capable of iteratively learning the hyperparamters as training data is collected, are required. Moreover, with the hyperparameters of each model fixed to same value LGPR is not ideally-suited to model non-stationary data.

To address these limitations, Wilcox and Yip \cite{wilcox2020solar} propose a variant of LGPR, called sparse online locally adaptive regression using Gaussian processes (SOLAR GP). Wilcox and Yip use the streaming sparse Gaussian process approximation framework developed by Bui et al. \cite{bui2017streaming} for each local model. This allows the sparse approximation of each model's posterior distribution and hyperparameters to be recursively updated as new data is collected. This allows for local models to have separate hyperparameters, which is ideal for modeling non-stationary data. Additionally, SOLAR GP defines a separate Gaussian process model called the \textit{base} model, which iteratively learns the hyperparameters of the similarity measure \ref{eq: weights}, as more data is collected. 

Common to both LGPR and SOLAR GP is that as new training data is collected, a decision is to be made as to whether the new data should be used to update an existing model or to instantiate a new one. The decision rule is based on the notion of similarity, meaning that we look for the model that is most similar, in some well-defined sense, to the new data and provided that model is sufficiently similar we update it. Otherwise, we conclude that no model is similar to the new data, and hence a new model should be instantiated. Ultimately, the creation of new models intrinsically relies on how similarity is defined. Both methods make the notion of similarity precise in terms of a covariance kernel, which reflects how far, in input space, new data is to an existing model. Thus, new data that is sufficiently far from all other existing models will give rise to a new model. 

In this paper, we propose a new method called Wasserstein-splitting Gaussian process regression WGPR. The primary innovation of our method is the use of a new definition of similarity based on the effect new data has on the predictive distribution of each existing model. Intuitively, if the new data does not significantly change a model's predictive distribution then we consider the new data to be similar to that model. We formalize this intuition in terms of the Wasserstein distance, a metric over distributions. To examine the influence of our new definition of similarity we compare the performance of WGPR to SOLAR GP on a 1-dimensional data set, as well as, several other publicly available data sets.

